Positron propagation in semi-relativistic plasmas: particle spectra and the annihilation line shape

By solving the Fokker-Planck equation directly we examine effects of annihilation, particle escape and injection on the form of a steady-state positron distribution in thermal hydrogen plasmas with $kT<m_ec^2$. We show that the escape of positrons in the form of electron-positron pairs and/or pair plasma has an effect on the positron distribution causing, in some cases, a strong deviation from a Maxwellian. Additionally, we present accurate formulas for energy exchange rates, and losses due to Coulomb scattering, bremsstrahlung, and Compton scattering in the Klein-Nishina regime. Suggesting that annihilation features observed by SIGMA telescope from Nova Muscae and the 1E 1740.7-2942 are due to the positron/electron slowing down and annihilation in thermal plasma, the electron number density and the size of the emitting regions have been estimated. We show that in the case of Nova Muscae the observed radiation is coming from a pair plasma stream ($n_{e^+}\approx n_{e^-}$) rather than from a gas cloud. We argue that two models are probably relevant to the 1E 1740.7-2942 source: annihilation in (hydrogen) plasma $n_{e^+}\la n_{e^-}$ at rest, and annihilation in the pair plasma stream, which involves matter from the source environment.

==> epsfig <==
#!/usr/local/bin/perl
#
# usage: epsfig [-c] FILE
#
# Write (possibly compressed) epsfig FILE to stdout.  The TEXINPUTS path is
# searched for FILE{,.gz,z,Z}.  With the -c option the FILE is gziped and
# FILE.bb is generated.  If FILE is in the system default $SYSTEXINPUTS path
# no attempt is made to epsbb it.
#
# Used by epsfig.sty inside backquoted dvips specials.
#
#  Author: Peter Whaite (peta@mcrcim.mcgill.edu)
#          Centre for Intelligent Machines, McGill University.
# $Id: epsfig,v 1.3 1993/09/13 22:55:00 peta Exp $

## USER CONFIG -- edit the following to suit your system.
#
$SYSTEXINPUTS='.:/usr/local/tex/lib/texinputs';
$ZCAT='/usr/local/bin/gunzip -c';
#
## END USER CONFIG

while ($_=shift,/^-/)
{
    /^-c/ && do {$compress++;next};
    die "$0: bad option $_\nusage: $0 [-c] <file>\n";
}
die "usage: $0 [-c] <file>\n" unless $#ARGV == -1;
$file=$_;

$TEXINPUTS=$ENV{'TEXINPUTS'};
$TEXINPUTS .= $SYSTEXINPUTS if ((! $TEXINPUTS)||($TEXINPUTS =~ /:$/));
@SYSTEXINPUTS = split(/:/,$SYSTEXINPUTS);
@TEXINPUTS = split(/:/,$TEXINPUTS);

foreach $dir (@TEXINPUTS)
{
    $epsf = "$dir/$file";
    (-f $epsf)      && do {$cmd = "$epsf"; $uncompressed=1; last;};
    (-f "$epsf.gz") && do {$cmd="$ZCAT $epsf|"; last;};
    (-f "$epsf.z")  && do {$cmd="$ZCAT $epsf|"; last;};
    (-f "$epsf.Z")  && do {$cmd= "$ZCAT $epsf|"; last;};
}
$cmd || die("$0: $file.{z,gz,Z} not found\n");

open(EPSF,$cmd) || die("$0: $cmd: $!\n");
while (<EPSF>)
{
    print;
}
close EPSF;

if ($compress && $uncompressed)
{
    exit(0) if (grep(/^$dir$/,@SYSTEXINPUTS) && ($dir =~ m#^/#));
    system("epsbb $epsf");
};

# Local Variables:
# mode: perl
# auto-fill-hook: do-auto-fill
# End:

